Inductive Graph Few-shot Class Incremental Learning

Node classification with Graph Neural Networks (GNN) under a fixed set of labels is well known in contrast to Graph Few-Shot Class Incremental Learning (GFSCIL), which involves learning a GNN classifier as graph nodes and classes growing over time sporadically. We introduce inductive GFSCIL that continually learns novel classes with newly emerging nodes while maintaining performance on old classes without accessing previous data. This addresses the practical concern of transductive GFSCIL, which requires storing the entire graph with historical data. Compared to the transductive GFSCIL, the inductive setting exacerbates catastrophic forgetting due to inaccessible previous data during incremental training, in addition to overfitting issue caused by label sparsity. Thus, we propose a novel method, called Topology-based class Augmentation and Prototype calibration (TAP). To be specific, it first creates a triple-branch multi-topology class augmentation method to enhance model generalization ability. As each incremental session receives a disjoint subgraph with nodes of novel classes, the multi-topology class augmentation method helps replicate such a setting in the base session to boost backbone versatility. In incremental learning, given the limited number of novel class samples, we propose an iterative prototype calibration to improve the separation of class prototypes. Furthermore, as backbone fine-tuning poses the feature distribution drift, prototypes of old classes start failing over time, we propose the prototype shift method for old classes to compensate for the drift. We showcase the proposed method on four datasets.

==> chapters/supplymentary.tex <==
\section*{Supplementary Material}

\section{Computational Complexity Analysis}
Overall, the complexity of the TAP method is linear with the number of graph edges and nodes, i.e. O($|E|+n$), maintaining a similar complexity to that of the GAT encoder (equivalent to GAT-finetune). 
Specifically, reviewing the three main components of TAP, the TMCA introduces additional complexity due to tripling the base training set size, resulting in a complexity of O($3|E|$). The IPSN and PSO components contribute to computing complexities of O($n_q*d$) and O($|\mathcal{C}^{\mathcal{T}-1}|*n_s*d$), respectively, where $n_q$ and $n_s$ are the number of novel query and support nodes, $d$ is the feature dimension and $|\mathcal{C}^{\mathcal{T}-1}|$ is the number of old classes.
Consequently, the additional complexity introduced by IPCN and PSO remains linear with the number of novel nodes, i.e. O($n$). Therefore, the overall extra computational burden is manageable. The training time comparison is presented in Table \ref{table:comput_time}, with experiments conducted on a Tesla $P100-SXM2-16GB$ GPU device, running 1000 epochs for the base training and 5 epochs on each incremental session.
%By comparison, the TAP method introduces the extra computing burdens from the triple-branch class augmentation, the prototype calibration for both old(PSO) and novel classes (IPCN). 
%IPSN entails computing the prototype using pseudo-labeled query nodes, causing O($n_q$*d) where $n_q$ is the number of query nodes at each session, and d is the feature dimension. While the PSO involves calculating the old prototype shift using similarities among old prototypes and the novel support set, it causes the complexity of O(N'*$n_s$*d), where N' is the number of old classes, $n_s$ is the number of novel support nodes. 

\begin{table}[!htbp]
\vspace{-0.3cm}
    \centering
    \caption{Training complexity comparison on the Amazon\_clothing dataset (5-way 5-shot).}
    \vspace{-0.2cm}
    \scalebox{0.9}{
    \begin{tabular}{ccccc}
         \toprule
         Methods & GAT-finetune  & GAT-frozen  & SAVC  & TAP \\
         \midrule
         Time(sec) & 114.9 & 110.8 & 217.2 & 230.0  \\
    \bottomrule
    \end{tabular}}
    \label{table:comput_time}
    \vspace{-0.3cm}
\end{table}

\section{Additional Validation of Class Augmentation}
\label{appendix:augment}
We provide additional TAP variants to further evaluate the effectiveness of class augmentation method in TAP as described below. 
\renewcommand{\labelenumi}{\roman{enumi}.}
\begin{enumerate}[leftmargin=0.6cm]
    \item TAP\_ED: Instead of the TMCA method, it applies the random edge drop method to generate the augmented classes;
    \item TAP\_FM: It utilizes the random feature mask method to generate the augmented class;
    \item TAP\_MED: It employs the graph mask method \cite{hou2022graphmae} to replace our augmentation method;
    \item TAP\_Diff: It applies the graph diffusion method \cite{gasteiger2019diffusion} for the class augmentation;
    \item TAP\_SC: It applies topology-free and topology-varying augmentation but doesn't change node labels, and remains the same class space; 
    % \item TAP\_FProj: It freezes the GAT backbone and only finetunes the appended projection layer;
\end{enumerate}

Their performance is presented in Table \ref{table:comp_ablation}. Compared with TAP, TAP\_ED, TAP\_FM, TAP\_MED, TAP\_Diff experienced 2.9\%, 1.4\%, 1.6\% and 1.2\% performance drop in the accuracy of the last session, respectively. 
The four variants do not help align the augmentation method with future tasks, thus failing to improve the model's generalization ability on novel classes. TAP\_SC regards the augmented data as a perturbation of existing data without changing the node labels. This disables the ``reserved space'' for distinct topologies of graphs of novel classes during base training, thereby leading to a suboptimal performance.  

\section{Generalizability for GNN backbones}
To evaluate the generalizability of TAP across various GNN backbones, we conducted experiments by replacing the GAT backbone with GCN \cite{kipf2016semi} and GraphSAGE \cite{hamilton2017inductive}. The results of these experiments are presented in Table \ref{table:ablation_gnn}. For comparison, we also report the performance of GNN-finetunes, GNN-frozen, and one representative baseline (SAVC). Overall, since the design of TAP is not dependent on a specific GNN architecture, it consistently outperforms other baselines, regardless of whether the GCN or GraphSAGE backbones are used. Specifically, TAP-GCN achieves a 4.5\% and 8.2\% improvement in performance over the SAVC-GCN and GCN-frozen baselines, respectively, in terms of last-session accuracy. Similarly, TAP-GraphSAGE surpasses these baselines by 1.5\% and 5.3\%, respectively. These results further validate the effectiveness of our method across different GNN backbones.

\section{Additional Ablation Study of New Perspective}

To further illustrate the effectiveness of each individual component, we conducted an additional ablation study in which each component is applied separately on top of the GAT backbone. Specifically:
\renewcommand{\labelenumi}{\roman{enumi}.}
\begin{enumerate}[leftmargin=0.6cm]
    \item TAP\_TFA: It exclusively employs topology-free augmentation based on the GAT-frozen training paradigm.
    \item TAP\_TVA: It exclusively employs topology-varying augmentation based on the GAT-frozen training paradigm.
    \item TAP\_PSO: It applies model adaptation and Prototype Shift for Old classes (PSO) on the GAT-finetune training paradigm.
    \item TAP\_IPCN: It applies model adaptation and Iterative Prototype Calibration for Novel classes (IPCN) based on the GAT-finetune training paradigm.
    \item TAP\_CE: It replaces the margin-based loss with the cross-entropy loss, equivalent to specifying  $\kappa\!=\!0$ for margin.
\end{enumerate}
Table~\ref{table:ablation_single} shows the ablations on the Amazon\_clothing and DBLP datasets. Overall, each component improves the accuracy in comparison to GAT-frozen and GAT-finetune, affirming their efficacy for inductive GFSCIL. Particularly, considering the accuracy in the last session, both class augmentation methods demonstrate approximately 1.7\% improvement on average compared with GAT-frozen. Model finetune with PSO can lead to 2.2\% performance improvement on average, while model finetune with IPCN can deliver the improvement of 3.7\% on average. TAP\_CE, compared with TAP, results in 1\% and 2.5\% performance drops because of replacing the margin-based loss with cross-entropy loss.
The combination of those components provides a comprehensive solution: TAP\_TFA and TAP\_TVA enhance the generalization ability on unseen classes and structural patterns, model finetuning with PSO allows the model to assimilate novel knowledge while preventing drift of old prototypes, and IPCN benefits the model in reducing the variance of novel prototypes and improving their representativeness. 

\begin{table*}[h]
    \centering
    \tabcolsep 3pt
    \caption{Performance comparison of different augmentation variants of TAP on the Amazon\_clothing dataset.}
    \vspace{-0.3cm}
    \scalebox{0.9}{
        \begin{tabular}{l c c c c c c c c c c c c}
             \toprule
              & \multicolumn{12}{c}{Amazon\_clothing (5-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & A/Acc. & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             TAP\_ED  &0.919 &0.864 &0.826 &0.777 &0.749 & 0.716 & 0.693 & 0.675 & 0.657 &0.639 & 0.751 & 0.280 \\
             TAP\_FM  &0.936 &0.889 &0.852 &0.803 &0.772 & 0.738 & 0.716 & 0.696 & 0.678 &0.654 & 0.774 & 0.282 \\
             TAP\_MED  &0.925&0.902&0.848&0.801&0.763&0.735&0.718&0.701&0.680&0.652&0.772&0.273 \\
             TAP\_Diff  &0.932&0.905&0.854&0.803&0.756&0.720&0.710&0.691&0.674&0.656&0.770&0.276 \\
             TAP\_SC  & 0.939 & 0.889 & 0.853 & 0.803 & 0.772 & 0.739 & 0.716 & 0.698 & 0.680 & 0.655 & 0.775 & 0.284 \\
             TAP &0.935 &0.889 &0.851 &0.804 &0.775 & 0.745 & 0.725 & 0.708 & 0.692 & 0.668 & 0.780 & 0.267  \\
             \bottomrule 
        \end{tabular}}
    \label{table:comp_ablation}
\end{table*}

\begin{table*}[!h]
\vspace{-0.1cm}
    \centering
    \tabcolsep 3pt
    \caption{Performance comparison on different GNN backbones of TAP on the Amazon\_clothing dataset.}
   \vspace{-0.3cm}
    \scalebox{0.9}{
        \begin{tabular}{lcccccccccccc}
             \toprule
              & \multicolumn{12}{c}{Amazon\_clothing (5-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & A/Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GCN\_finetune  &0.941&0.096&0.064&0.069&0.133&0.148&0.061&0.087&0.053&0.059&0.171&0.882  \\
             GCN\_frozen  &0.943&0.838&0.771&0.691&0.645&0.592&0.551&0.519&0.490&0.467&0.651&0.476 \\            
             GCN\_SAVC  &0.937&0.906&0.854&0.797&0.724&0.653&0.606&0.573&0.534&0.505&0.694&0.421 \\
             GCN\_TAP &0.941&0.856&0.803&0.739&0.696&0.651&0.616&0.589&0.568&0.549&0.701&0.396 \\
            \midrule
             & \multicolumn{12}{c}{Amazon\_clothing (5-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & A/Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GraphSAGE\_finetune  &0.957&0.088&0.079&0.078&0.139&0.138&0.072&0.108&0.061&0.058&0.178&0.899 \\
             GraphSAGE\_frozen  &0.959&0.867&0.779&0.703&0.641&0.579&0.541&0.504&0.481&0.458&0.651&0.500 \\            
             GraphSAGE\_SAVC &0.958&0.905&0.813&0.750&0.688&0.631&0.591&0.553&0.522&0.496&0.691&0.462 \\
             GraphSAGE\_TAP &0.961&0.910&0.846&0.791&0.712&0.637&0.620&0.576&0.537&0.511&0.710&0.450 \\
             \bottomrule 
        \end{tabular}}
    \label{table:ablation_gnn}
    \vspace{-0.1cm}
\end{table*}

\begin{table*}[t]
\vspace{-0.1cm}
    \centering
    \tabcolsep 3pt
    \caption{Additional Ablation studies of TAP on the Amazon\_clothing dataset.}
   \vspace{-0.3cm}
    \scalebox{0.9}{
        \begin{tabular}{lcccccccccccc}
             \toprule
              & \multicolumn{12}{c}{Amazon\_clothing (5-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & A/Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.930 &0.121 &0.087 &0.103 &0.087 & 0.088 & 0.092 & 0.069 & 0.058 &0.064 & 0.170 & 0.867  \\
             GAT\_frozen  &0.931 &0.861 &0.817 &0.756 &0.721 & 0.685 & 0.656 & 0.636 & 0.617 &0.591 & 0.727 & 0.340  \\
             \midrule
             TAP\_TFA  &0.927 &0.872 &0.824 &0.769 &0.736 & 0.699 & 0.671 & 0.648 & 0.628 &0.602 & 0.738 & 0.326 \\
             TAP\_TVA  &0.925 &0.860 &0.816 &0.761 &0.728 & 0.696 & 0.669 & 0.648 & 0.631 &0.606 & 0.734 & 0.319  \\
             TAP\_PSO  &0.945 &0.883 &0.839 &0.780 &0.746 & 0.713 & 0.687 & 0.669 & 0.651 &0.624 & 0.754 & 0.321  \\
             TAP\_IPCN  &0.931 &0.878 &0.837 &0.783 &0.752 & 0.726 & 0.700 & 0.679 & 0.662 & 0.641 & 0.759 & 0.289  \\
             TAP\_CE  &0.919 &0.870 &0.836 &0.791 &0.764 & 0.736 & 0.714 & 0.695 & 0.677 &0.658 & 0.766 & 0.261  \\
             TAP &0.935 &0.889 &0.851 &0.804 &0.775 & 0.745 & 0.725 & 0.708 & 0.692 & 0.668 & 0.780 & 0.267  \\
            \midrule
            \midrule
            & \multicolumn{12}{c}{DBLP (10-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & A/Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.637 &0.051 &0.054 &0.049 &0.044 & 0.038 & 0.036 & 0.035 & 0.031 & 0.033 & 0.101 & 0.603  \\
             GAT\_frozen  &0.633 &0.605 & 0.582 & 0.559 & 0.536 & 0.514 & 0.498 & 0.482 & 0.467 & 0.455 & 0.533 & 0.178 \\
             \midrule
             TAP\_TFA  &0.606 &0.599 &0.585 &0.568 &0.550 & 0.534 & 0.518 & 0.506 & 0.491 &0.481 & 0.544 & 0.125 \\
             TAP\_TVA  &0.617 &0.599 &0.581 &0.563 &0.544 & 0.527 & 0.512 & 0.499 & 0.484 &0.474 & 0.540 & 0.143 \\
             TAP\_PSO  &0.657 &0.628 &0.603 &0.579 &0.554& 0.531 & 0.513 & 0.496 & 0.477 & 0.465 & 0.550 & 0.193  \\
             TAP\_IPCN  &0.634 &0.609 &0.589 &0.569 &0.550& 0.531 & 0.517 & 0.503 & 0.489 & 0.479 & 0.547 & 0.156 \\
             TAP\_CE  &0.613 &0.599 &0.582 &0.568 &0.551 & 0.532 & 0.515 & 0.501 & 0.486 &0.478 & 0.542 & 0.135  \\
             TAP &0.641 &0.631 &0.612 &0.594 &0.577 & 0.557 & 0.540 & 0.525 & 0.510 & 0.503 & 0.569 & 0.138  \\
             \bottomrule 
        \end{tabular}}
    \label{table:ablation_single}
    \vspace{-0.1cm}
\end{table*}

\begin{table*}[th]
\vspace{-0.1cm}
    \centering
    \tabcolsep 3pt
    \caption{Performance comparison on the N-way 1-shot setting over different datasets.}
   \vspace{-0.3cm}
    \scalebox{0.9}{
        \begin{tabular}{lcccccccccccc}
             \toprule
              & \multicolumn{12}{c}{Obgn-arxiv (3-way 1-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & A/Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.668&0.482&0.270&0.183&0.141&0.089&0.081&0.084&0.061&0.056 &0.211 &0.612  \\
             GAT\_frozen  &0.662&0.579&0.538&\underline{0.491}&0.437&0.414&0.392&\underline{0.362}&0.346&0.323&0.454 &0.339 \\
             CLOM\cite{zou2022margin} &0.654&0.576&0.532&0.481&0.427&0.402&0.383&0.353&0.340&0.316 &0.446 &\underline{0.338} \\
             LCWOF\cite{kukleva2021generalized} &0.666&0.586&0.544&0.489&0.435&0.411&0.391&\underline{0.362}&\underline{0.348}&\underline{0.324}&\underline{0.455} &0.341   \\
             % Alice\cite{peng2022few}  &0.654&0.572&0.537&0.487&0.434&0.406&0.386&0.345&0.332&0.310 &0.446 &0.344 \\
             SAVC\cite{song2023learning}  &\textbf{0.674}&\underline{0.589}&\underline{0.549}&0.490&\underline{0.439}&\underline{0.416}&\underline{0.393}&0.349&0.336&0.313 &0.454 &0.361 \\
             NC-FSCIL\cite{yang2023neural} &0.658&0.490&0.395&0.391&0.384&0.360&0.331&0.303&0.292&0.287 &0.389 &0.371\\
             Geometer\cite{peng2022few} &0.661&0.579&0.538&\underline{0.491}&0.437&0.414&0.392&0.361&0.346&0.323 &{0.454} &0.338\\
             \rowcolor{LightCyan} \textbf{TAP} &\underline{0.669}&\textbf{0.599}&\textbf{0.565}&\textbf{0.513}&\textbf{0.462}&\textbf{0.433}&\textbf{0.410}&\textbf{0.378}&\textbf{0.366}&\textbf{0.344} &\textbf{0.474} &\textbf{0.325} \\
            \midrule
             & \multicolumn{12}{c}{Amazon\_clothing (5-way 1-shot)}\\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & A/Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.931&0.082&0.061&0.026&0.051&0.078&0.091&0.056&0.037&0.022 &0.143 &0.909\\
             GAT\_frozen  &0.931&0.825&0.778&0.714&0.669&0.612&0.574&0.552&0.531&0.511 &0.669 &0.420\\
             CLOM\cite{zou2022margin}  &0.943&\underline{0.836}&0.775&0.723&0.674&0.615&0.578&0.555&0.533&0.511 &0.675 &0.432 \\
             LCWOF\cite{kukleva2021generalized} &0.931&0.817&0.766&0.707&0.658&0.603&0.567&0.544&0.523&0.500  &0.662 &0.431\\
             % Alice\cite{peng2022few}  &0.935&0.832&0.778&0.729&\underline{0.677}&0.620&0.582&0.555&0.535&0.513 &0.675 &0.422 \\
             SAVC\cite{song2023learning}  &0.924&0.836&0.778&\underline{0.735}&\underline{0.677}&\underline{0.621}&0.585&0.558&0.535&0.518 &0.677 &\underline{0.406}\\
             NC-FSCIL\cite{yang2023neural} &0.835&0.709&0.622&0.580&0.504&0.479&0.426&0.424&0.427&0.372&0.538 &0.463\\
             Geometer\cite{peng2022few} &\textbf{0.944}&0.832&\underline{0.781}&0.720&\underline{0.677}&0.619&\underline{0.589}&\underline{0.566}&\underline{0.545}&\underline{0.520} &\underline{0.679} &0.423\\
             \rowcolor{LightCyan} \textbf{TAP} &\underline{0.934}&\textbf{0.837}&\textbf{0.783}&\textbf{0.743}&\textbf{0.703}&\textbf{0.652}&\textbf{0.629}&\textbf{0.605}&\textbf{0.585}&\textbf{0.565} &\textbf{0.703} &\textbf{0.369}\\
             \midrule             
             & \multicolumn{12}{c}{DBLP (10-way 1-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions}\\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & A/Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.638&0.225&0.113&0.089&0.073&0.065&0.054&0.051&0.043&0.041 &0.139 &0.597 \\
             GAT\_frozen  &0.632&0.595&0.567&0.540&0.512&0.485&0.464&0.444&0.426&0.412 &0.507 &0.220 \\
             CLOM\cite{zou2022margin}  &0.645&0.607&0.575&0.544&0.516&0.489&0.468&0.448&0.432&0.417 &0.514 &0.228 \\
             LCWOF\cite{kukleva2021generalized}  &0.628&0.591&0.559&0.531&0.503&0.478&0.457&0.437&0.420&0.408 &0.501 &0.220 \\
             Alice\cite{peng2022few}  &0.616&0.590&0.563&0.536&0.514&0.490&0.471&0.453&\underline{0.436}&0.422 &0.509 &0.194 \\
             SAVC\cite{song2023learning}  &0.608&0.589&0.564&0.541&0.518&\underline{0.495}&\underline{0.473}&\underline{0.454}&\underline{0.436}&\underline{0.423} &0.509 &\underline{0.185} \\
             NC-FSCIL\cite{yang2023neural} &0.430&0.319&0.296&0.298&0.282&0.277&0.286&0.260&0.244&0.243&0.293 &0.187\\
             Geometer\cite{peng2022few} &\textbf{0.653}&\underline{0.613}&\underline{0.579}&\underline{0.547}&\underline{0.519}&0.491&0.469&0.447&0.428&0.415 &\underline{0.516} &0.238\\
             \rowcolor{LightCyan} \textbf{TAP} &\underline{0.642}&\textbf{0.616}&\textbf{0.592}&\textbf{0.567}&\textbf{0.545}&\textbf{0.522}&\textbf{0.501}&\textbf{0.486}&\textbf{0.469}&\textbf{0.459}  &\textbf{0.540} &\textbf{0.183}\\
            \midrule
             & \multicolumn{12}{c}{Cora\_full (5-way 1-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions}\\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9  & A/Acc.  & PD \textcolor{red}{$\downarrow$}  \\
             \midrule
             GAT\_finetune  &0.937&0.104&0.075&0.052&0.051&0.047&0.042&0.039&0.041&0.036 &0.142 &0.901\\
             GAT\_frozen  &\textbf{0.946}&0.813&\underline{0.711}&\underline{0.645}&{0.567}&0.529&0.487&{0.455}&0.426&0.401 &0.598 &0.544\\
             CLOM\cite{zou2022margin}  &0.943&0.812&\underline{0.711}&0.641&\underline{0.572}&\underline{0.532}&\underline{0.490}&\underline{0.458}&0.432&0.402 &\underline{0.599} &0.540\\
             LCWOF\cite{kukleva2021generalized} &0.938&0.799&0.695&0.625&0.554&0.511&0.473&0.445&0.420&0.392 &0.585 &0.545\\
             % Alice\cite{peng2022few}  &0.941&0.796&0.691&0.625&0.558&0.516&0.472&0.445&0.420&0.394 &0.586 &0.546\\
             SAVC\cite{song2023learning}  &0.939&0.786&0.680&0.607&0.539&0.499&0.458&0.430&0.405&0.375 &0.571 &0.564\\
             NC-FSCIL\cite{yang2023neural} &0.897&0.672&0.632&0.575&0.507&0.466&0.438&0.417&0.397&0.366 &0.537 &0.531\\
             Geometer\cite{peng2022few} &0.938& \underline{0.815}& {0.697}& 0.631& 0.567& 0.531& 0.486& 0.452& \underline{0.435}& \underline{0.411} &0.596 &\underline{0.526}\\
             \rowcolor{LightCyan} \textbf{TAP} &\underline{0.944}&\textbf{0.838}&\textbf{0.747}&\textbf{0.682}&\textbf{0.621}&\textbf{0.579}&\textbf{0.538}&\textbf{0.506}&\textbf{0.480}&\textbf{0.450} &\textbf{0.638} &\textbf{0.493}\\
             \bottomrule 
        \end{tabular}}
    \label{table:1-shot}
\end{table*}

\begin{table*}[h]
% \vspace{-0.3cm}
    \centering
    \caption{Performance comparison with regard to varying number of sessions on the Amazon\_clothing dataset (3-way 5-shot).}
    % \vspace{-0.2cm}
    \scalebox{0.9}{
    \begin{tabular}{ccccc|cccc|cccc}
         \toprule
        & \multicolumn{4}{c}{All classes} &\multicolumn{4}{c}{Base classes} &\multicolumn{4}{c}{Novel classes} \\
        \cline{2-13} 
        & \multicolumn{12}{c}{Number of total sessions (\#)} \\
        \cline{2-13} 
         Methods & \#5  & \#10  & \#15  & \#20 & \#5  & \#10  & \#15  & \#20 & \#5  & \#10  & \#15  & \#20 \\
         \midrule
         GAT-frozen &0.762&0.703&0.680&0.545 &0.812&0.847&0.849&0.903 &0.473&0.478&0.516&0.439 \\
         SAVC & 0.780 & 0.738 & 0.652 & 0.539 & 0.805 & 0.839 & 0.845 & 0.914 &0.592 & 0.554 & 0.508 & 0.428  \\
         TAP &0.781&0.747&0.719&0.632 &0.811&0.846&0.827&0.862 &0.553&0.593&0.639&0.563 \\
    \bottomrule
    \end{tabular}}
    \label{table:perf_session}
    \vspace{-0.3cm}
\end{table*}

\begin{table*}[h]
% \vspace{-0.3cm}
    \centering
    \caption{Performance relation to dataset statistics w.r.t. average degree and homophily rate.}
    \vspace{-0.2cm}
    \scalebox{0.9}{
    \begin{tabular}{ccccc}
         \toprule
         Methods & Amazon\_clothing  & DBLP  & Cora\_full  & Ogbn-arxiv \\
         \midrule
         Average degree & 7.35 & 14.14 & 6.59 & 13.7  \\
         Homophily rate & 0.62 & 0.29 & 0.59 & 0.72  \\
         Improvements & 7.7\% & 4.8\% & 7.0\% & 5.8\%  \\
    \bottomrule
    \end{tabular}}
    \label{table:perf_stats}
    \vspace{-0.3cm}
\end{table*}

\section{Experiments on N-way 1-shot Setting}
\label{appendix:1-shot}
%To further elaborate on the performance of TAP on the N-way 1-shot setting, we provide specific experimental results in Table \ref{table:1-shot} as the complementary for Figure \ref{fig:1-shot} in Section \ref{sec:1-shot}. As observed in the table, in terms of the last session accuracy, TAP achieves improvements of 2.0\%, 4.5\%, 3.6\% and 3.9\% on Ogbn-arxiv, Amazon\_clothing, DBLP and Cora\_full, respectively, compared with the best baselines. The stable performance improvements demonstrate the strong robustness of TAP against the overfitting risk caused by the extremely label-sparsity problem.
To further elaborate on TAP’s performance in the N-way 1-shot setting, we present specific experimental results in Table \ref{table:1-shot}, which complement Figure \ref{fig:1-shot} in Section \ref{sec:1-shot}. As shown in the table, TAP achieves improvements of 2.0\%, 4.5\%, 3.6\%, and 3.9\% in the final session accuracy on the Ogbn-Arxiv, Amazon\_Clothing, DBLP, and Cora\_Full datasets, respectively, compared to the best baselines. These consistent performance improvements demonstrate TAP’s strong robustness against the overfitting risk associated with extreme label sparsity.

\section{Generalizability for Session Size}
To evaluate the impact of session size on TAP's performance, we conducted experiments varying the number of incremental sessions from 5 to 20. To deepen our understanding of this effect, we present the last session accuracy across base classes, novel classes, and all classes in Table \ref{table:perf_session}, respectively. The results reveal a strengthening trend in TAP's overall performance, with gains of 1.9\%, 4.4\%, 3.9\%, and 8.7\% over GAT-frozen as the number of sessions increases. For the base classes, GAT-frozen, which maintains a fixed backbone, slightly outperforms TAP. However, in the novel classes, TAP demonstrates significant improvements of 8\%, 11.5\%, 12.3\%, and 12.4\% over GAT-frozen. This indicates that TAP favors enhanced performance in extended sessions. Notably, TAP consistently achieves stable performance gains in novel classes regardless of session size.
When the number of sessions is limited, the prevalence of base classes in the test set tends to dominate overall performance. Conversely, as the number of sessions increases, the contribution of novel classes to the final performance becomes more significant, thereby highlighting TAP's advantage.

\section{Performance Relation to the Structural Statistics}
Table \ref{table:perf_stats} presents the potential influence of dataset statistics on model performance. It summarizes TAP's improvements of the last session accuracy over GAT\_frozen, alongside key dataset characteristics, \ie average node degree and graph homophily rate. The benchmark datasets exhibit a range of statistics, with edge density varying from 6.59 to 14.14 and homophily rates ranging from 0.29 to 0.72. Considering both performance and dataset statistical properties, TAP demonstrates strong robustness and generalizability, maintaining consistent performance across diverse datasets. Specifically, TAP does not show evident sensitivity on the average node degree, but it is more likely to achieve superior results on datasets with higher homophily rates, as evidenced by over 7.0\% improvements on Amazon\_clothing and Cora\_full compared to 4.8\% on DBLP. 


==> chapters/supplymentary_backup.tex <==
\section*{Supplementary Material}

\section{Additional Validation of Class Augmentation}

We provide additional TAP variants to further evaluate the effectiveness of class augmentation method in TAP as described below. 
%In particular, TAP\_ED, TAP\_FM, TAP\_ME, TAP\_Diff, TAP\_SC are five different augmentation methods, which are designed to validate the effectiveness of our TMCA. While TAP\_FProj freezes the GNN backbone and finetunes the appended projection layer to adapt novel classes, established to reveal the necessity of our finetuning method: 
\vspace{-0.1cm}
\renewcommand{\labelenumi}{\roman{enumi}.}
\begin{enumerate}[leftmargin=0.6cm]
    \item TAP\_ED: Instead of the TMCA method, it applies the random edge drop method to generate the augmented classes;
    \item TAP\_FM: It utilizes the random feature mask method to generate the augmented class;
    \item TAP\_MED: It employs the graph mask and reconstruction method \cite{hou2022graphmae} to replace our augmentation method;
    \item TAP\_Diff: It applies the graph diffusion method \cite{gasteiger2019diffusion} for the class augmentation;
    \item TAP\_SC: It applies topology-free and topology-varying augmentation but doesn't change node labels, and remains the same class space; 
    % \item TAP\_FProj: It freezes the GAT backbone and only finetunes the appended projection layer;
\end{enumerate}

Their performance is presented in Table \ref{table:comp_ablation}. Compared with TAP, TAP\_ED, TAP\_FM, TAP\_MED, TAP\_Diff experienced 2.9\%, 0.8\%, 1.4\% and 0.7\% performance drop in the accuracy of the last session, respectively. 
The four variants do not help align the augmentation method with future tasks, thus failing to improve the model's generalization ability on novel classes. TAP\_SC regards the augmented data as a perturbation of existing data without changing the node labels. This disables the ``reserved space'' for distinct topologies of graphs of novel classes during base training, thereby leading to a suboptimal performance.  

\begin{table*}[h]
    \centering
    \tabcolsep 3pt
    \caption{Performance comparison of different augmentation variants of TAP on Amazon\_clothing. Performance Drop (PD): difference between the accuracy on the first \vs last session.}
    \vspace{-0.3cm}
    \scalebox{0.6}{
        \begin{tabular}{lcccccccccccc}
             \toprule
              & \multicolumn{12}{c}{Amazon\_clothing (5-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc. & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             TAP\_ED  &0.919 &0.864 &0.826 &0.777 &0.749 & 0.716 & 0.693 & 0.675 & 0.657 &0.639 & 0.751 & 0.279 \\
             TAP\_FM  &0.936 &0.889 &0.852 &0.803 &0.772 & 0.738 & 0.716 & 0.696 & 0.678 &0.654 & 0.774 & 0.276 \\
             TAP\_MED  &0.925&0.902&0.848&0.801&0.763&0.735&0.718&0.701&0.680&0.652&0.772&0.271 \\
             TAP\_Diff  &0.932&0.905&0.854&0.803&0.756&0.720&0.710&0.691&0.674&0.656&0.770&0.274 \\
             TAP\_SC  & 0.939 & 0.889 & 0.853 & 0.803 & 0.772 & 0.739 & 0.716 & 0.698 & 0.680 & 0.655 & 0.775 & 0.289 \\
             TAP &0.935 &0.889 &0.851 &0.804 &0.775 & 0.745 & 0.725 & 0.708 & 0.692 & 0.668 & 0.780 & 0.264  \\
             \bottomrule 
        \end{tabular}}
    \label{table:comp_ablation}
\end{table*}

\section{Computational Complexity Analysis}
Overall, the complexity of the TAP method is linear with the number of graph edges and nodes, i.e. O($|E|+n$), maintaining a similar complexity to that of the GAT encoder (equivalent to GAT-finetune). 
Specifically, reviewing the three main components of TAP, the TMCA introduces additional complexity due to tripling the base training set size, resulting in a complexity of O($3|E|$). The IPSN and PSO components contribute to computing complexities of O($n_q*d$) and O($|\mathcal{C}^{\mathcal{T}}|*n_s*d$), respectively, where $n_q$ and $n_s$ are the number of novel query and support nodes, $d$ is the feature dimension and $|\mathcal{C}^{\mathcal{T}}|$ is the number of old classes.
Consequently, the additional complexity introduced by IPCN and PSO remains linear with the number of novel nodes, i.e. O($n$). Therefore, the overall extra computational burden is manageable. The training time comparison is presented below, with experiments conducted on a Tesla $P100-SXM2-16GB$ GPU device, running 1000 epochs for the base training and 5 epochs on each incremental session:
%By comparison, the TAP method introduces the extra computing burdens from the triple-branch class augmentation, the prototype calibration for both old(PSO) and novel classes (IPCN). 
%IPSN entails computing the prototype using pseudo-labeled query nodes, causing O($n_q$*d) where $n_q$ is the number of query nodes at each session, and d is the feature dimension. While the PSO involves calculating the old prototype shift using similarities among old prototypes and the novel support set, it causes the complexity of O(N'*$n_s$*d), where N' is the number of old classes, $n_s$ is the number of novel support nodes. 

\begin{table}[!htbp]
\vspace{-0.3cm}
    \centering
    \caption{Training complexity comparison on the Amazon\_clothing dataset (5-way 5-shot).}
    \vspace{-0.2cm}
    \scalebox{0.8}{
    \begin{tabular}{ccccc}
         \toprule
         Methods & GAT-finetune  & GAT-frozen  & SAVC  & TAP \\
         \midrule
         Time(sec) & 114.9 & 110.8 & 217.2 & 230.0  \\
    \bottomrule
    \end{tabular}}
    \label{table:comput_time}
    \vspace{-0.3cm}
\end{table}

\section{Generalizability for GNN backbones}
To evaluate the generalizability of TAP across various GNN backbones, we conducted experiments by replacing the GAT backbone with GCN \cite{kipf2016semi} and GraphSAGE \cite{hamilton2017inductive}. The results of these experiments are presented in Table \ref{table:ablation_gnn}. For comparison, we also report the performance of GNN-finetunes, GNN-frozen, and the representative baseline (SAVC). Overall, since the design of TAP is not dependent on a specific GNN architecture, it consistently outperforms other baselines, regardless of whether the GCN or GraphSAGE backbones are used. Specifically, TAP-GCN achieves a 4.5\% and 8.2\% improvement in performance over the SAVC-GCN and GCN-frozen baselines, respectively, in terms of last-session accuracy. Similarly, TAP-GraphSAGE surpasses these baselines by 1.5\% and 5.3\%, respectively. These results further validate the effectiveness of our method across different GNN backbones.

\begin{table*}[!h]
\vspace{-0.1cm}
    \centering
    \tabcolsep 3pt
    \caption{Performance comparison on different GNN backbones of TAP on the Amazon\_clothing dataset.}
   \vspace{-0.3cm}
    \scalebox{0.6}{
        \begin{tabular}{lcccccccccccc}
             \toprule
              & \multicolumn{12}{c}{Amazon\_clothing (5-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GCN\_finetune  &0.941&0.096&0.064&0.069&0.133&0.148&0.061&0.087&0.053&0.059&0.171&0.882  \\
             GCN\_frozen  &0.943&0.838&0.771&0.691&0.645&0.592&0.551&0.519&0.490&0.467&0.651&0.476 \\            
             GCN\_SAVC  &0.937&0.906&0.854&0.797&0.724&0.653&0.606&0.573&0.534&0.505&0.694&0.421 \\
             GCN\_TAP &0.941&0.856&0.803&0.739&0.696&0.651&0.616&0.589&0.568&0.549&0.701&0.396 \\
            \midrule
             & \multicolumn{12}{c}{Amazon\_clothing (5-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GraphSAGE\_finetune  &0.957&0.088&0.079&0.078&0.139&0.138&0.072&0.108&0.061&0.058&0.178&0.899 \\
             GraphSAGE\_frozen  &0.959&0.867&0.779&0.703&0.641&0.579&0.541&0.504&0.481&0.458&0.651&0.500 \\            
             GraphSAGE\_SAVC &0.958&0.905&0.813&0.750&0.688&0.631&0.591&0.553&0.522&0.496&0.691&0.462 \\
             GraphSAGE\_TAP &0.961&0.910&0.846&0.791&0.712&0.637&0.620&0.576&0.537&0.511&0.710&0.450 \\
             \bottomrule 
        \end{tabular}}
    \label{table:ablation_gnn}
    \vspace{-0.1cm}
\end{table*}


\section{Additional Ablation Studies}


% It is noticeable that TAP-PSO has the largest performance degradation by 4.8\%, which highlights the indispensable role of PSO. 
To further illustrate the effectiveness of each individual component, we conducted an additional ablation study in which each component was applied separately on top of the GAT backbone. Specifically:
\renewcommand{\labelenumi}{\roman{enumi}.}
\begin{enumerate}[leftmargin=0.6cm]
    \item TAP\_TFA: It exclusively employs topology-free augmentation based on the GAT-frozen training paradigm.
    \item TAP\_TVA: It exclusively employs topology-varying augmentation based on the GAT-frozen training paradigm.
    \item TAP\_PSO: It applies model adaptation and Prototype Shift for Old classes (PSO) on the GAT-finetune training paradigm.
    \item TAP\_IPCN: It applies model adaptation and Iterative Prototype Calibration for Novel classes (IPCN) based on the GAT-finetune training paradigm.
    \item TAP\_CE: It replaces the margin-based loss with the cross-entropy loss, equivalent to specifying  $\kappa\!=\!0$ for margin.
\end{enumerate}
Table~\ref{table:ablation_single} shows the ablations on Amazon\_clothing and DBLP. Overall, each component improves the accuracy in comparison to GAT-frozen and GAT-finetune, affirming their efficacy for inductive GFSCIL. Particularly, considering the accuracy in the last session, both class augmentation methods demonstrate approximately 1.7\% improvement on average compared with GAT-frozen. Model finetune with PSO can lead to 2.2\% performance improvement on average, while model finetune with IPCN can deliver the improvement of 3.7\%. TAP\_CE, compared with TAP, results in 1\% and 2.5\% performance drops because of replacing the margin-based loss with cross-entropy loss.
The combination of those components provides a comprehensive solution: TAP\_TFA and TAP\_TVA enhance the generalization ability on unseen classes and structural patterns, model finetuning with PSO allows the model to assimilate novel knowledge while preventing drift of old prototypes, and IPCN benefits the model in reducing the variance of novel prototypes and improving their representativeness. 



\begin{table*}[t]
\vspace{-0.1cm}
    \centering
    \tabcolsep 3pt
    \caption{Additional Ablation studies of TAP on the Amazon\_clothing dataset.}
   \vspace{-0.3cm}
    \scalebox{0.6}{
        \begin{tabular}{lcccccccccccc}
             \toprule
              & \multicolumn{12}{c}{Amazon\_clothing (5-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.930 &0.121 &0.087 &0.103 &0.087 & 0.088 & 0.092 & 0.069 & 0.058 &0.064 & 0.170 & 0.867  \\
             GAT\_frozen  &0.931 &0.861 &0.817 &0.756 &0.721 & 0.685 & 0.656 & 0.636 & 0.617 &0.591 & 0.727 & 0.340  \\
             \midrule
             TAP\_TFA  &0.927 &0.872 &0.824 &0.769 &0.736 & 0.699 & 0.671 & 0.648 & 0.628 &0.602 & 0.738 & 0.326 \\
             TAP\_TVA  &0.925 &0.860 &0.816 &0.761 &0.728 & 0.696 & 0.669 & 0.648 & 0.631 &0.606 & 0.734 & 0.319  \\
             TAP\_PSO  &0.945 &0.883 &0.839 &0.780 &0.746 & 0.713 & 0.687 & 0.669 & 0.651 &0.624 & 0.754 & 0.321  \\
             TAP\_IPCN  &0.931 &0.878 &0.837 &0.783 &0.752 & 0.726 & 0.700 & 0.679 & 0.662 & 0.641 & 0.759 & 0.289  \\
             TAP\_CE  &0.919 &0.870 &0.836 &0.791 &0.764 & 0.736 & 0.714 & 0.695 & 0.677 &0.658 & 0.766 & 0.261  \\
             TAP &0.935 &0.889 &0.851 &0.804 &0.775 & 0.745 & 0.725 & 0.708 & 0.692 & 0.668 & 0.780 & 0.264  \\
            \midrule
            \midrule
            & \multicolumn{12}{c}{DBLP (10-way 5-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.637 &0.051 &0.054 &0.049 &0.044 & 0.038 & 0.036 & 0.035 & 0.031 & 0.033 & 0.101 & 0.603  \\
             GAT\_frozen  &0.633 &0.605 & 0.582 & 0.559 & 0.536 & 0.514 & 0.498 & 0.482 & 0.467 & 0.455 & 0.533 & 0.178 \\
             \midrule
             TAP\_TFA  &0.606 &0.599 &0.585 &0.568 &0.550 & 0.534 & 0.518 & 0.506 & 0.491 &0.481 & 0.544 & 0.125 \\
             TAP\_TVA  &0.617 &0.599 &0.581 &0.563 &0.544 & 0.527 & 0.512 & 0.499 & 0.484 &0.474 & 0.540 & 0.143 \\
             TAP\_PSO  &0.657 &0.628 &0.603 &0.579 &0.554& 0.531 & 0.513 & 0.496 & 0.477 & 0.465 & 0.550 & 0.193  \\
             TAP\_IPCN  &0.634 &0.609 &0.589 &0.569 &0.550& 0.531 & 0.517 & 0.503 & 0.489 & 0.479 & 0.547 & 0.156 \\
             TAP\_CE  &0.613 &0.599 &0.582 &0.568 &0.551 & 0.532 & 0.515 & 0.501 & 0.486 &0.478 & 0.542 & 0.135  \\
             TAP &0.641 &0.631 &0.612 &0.594 &0.577 & 0.557 & 0.540 & 0.525 & 0.510 & 0.503 & 0.569 & 0.138  \\
             \bottomrule 
        \end{tabular}}
    \label{table:ablation_single}
    \vspace{-0.1cm}
\end{table*}




% \section{More Few-shot Settings}
% To validate the robustness and generalization ability of TAP on extreme label constraints, we provide the experimental results on the 1-shot setting, where only one label per class is given for training in the incremental session. 
% \begin{table*}[th]
% \vspace{-0.1cm}
%     \centering
%     \tabcolsep 3pt
%     \caption{Performance comparison on different few-shot settings of TAP on Amazon\_clothing.}
%    % \vspace{-0.3cm}
%     \scalebox{0.9}{
%         \begin{tabular}{lcccccccccccc}
%              \toprule
%               & \multicolumn{12}{c}{Obgn-arxiv (3-way 1-shot)} \\
%              \cline{2-13} 
%              Method & \multicolumn{12}{c}{Sessions} \\
%              \cline{2-13} 
%               &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
%              \midrule
%              GAT\_finetune  &0.668&0.482&0.270&0.183&0.141&0.089&0.081&0.084&0.061&0.056&0.212&0.612  \\
%              GAT\_frozen  &0.662&0.579&0.538&0.491&0.437&0.414&0.392&0.362&0.346&0.323&0.454&0.338  \\          
%              SAVC  &0.674&0.589&0.549&0.490&0.439&0.416&0.393&0.349&0.336&0.313&0.455&0.361  \\
%              TAP &0.669&0.599&0.565&0.513&0.462&0.433&0.410&0.378&0.366&0.344&0.474&0.325  \\
%             \midrule
%              & \multicolumn{12}{c}{Amazon\_clothing (5-way 1-shot)} \\
%              \cline{2-13} 
%              Method & \multicolumn{12}{c}{Sessions} \\
%              \cline{2-13} 
%               &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
%              \midrule
%              GAT\_finetune  &0.931&0.082&0.061&0.026&0.051&0.078&0.091&0.056&0.037&0.022&0.143&0.909 \\
%              GAT\_frozen  &0.931&0.825&0.778&0.714&0.669&0.612&0.574&0.552&0.531&0.511&0.669&0.420 \\            
%              SAVC  &0.924&0.836&0.778&0.735&0.677&0.621&0.585&0.558&0.535&0.518&0.677&0.406 \\
%              TAP &0.934&0.827&0.783&0.743&0.703&0.652&0.629&0.605&0.585&0.565&0.703&0.369 \\
%              \midrule
%              & \multicolumn{12}{c}{DBLP (10-way 1-shot)} \\
%              \cline{2-13} 
%              Method & \multicolumn{12}{c}{Sessions} \\
%              \cline{2-13} 
%               &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
%              \midrule
%              GAT\_finetune  &0.638&0.225&0.113&0.089&0.073&0.065&0.054&0.051&0.043&0.041&0.139&0.597  \\
%              GAT\_frozen  &0.632&0.595&0.567&0.540&0.512&0.485&0.464&0.444&0.426&0.412&0.508&0.220  \\          
%              SAVC  &0.603&0.589&0.564&0.541&0.518&0.495&0.473&0.454&0.436&0.422&0.510&0.181  \\
%              TAP &0.642&0.616&0.592&0.567&0.545&0.522&0.501&0.486&0.469&0.459&0.540&0.183  \\
%              \bottomrule 
%         \end{tabular}}
%     \label{table:1-shot}
%     \vspace{-0.1cm}
% \end{table*}


% \midrule
%              & \multicolumn{12}{c}{Amazon\_clothing (3-way 3-shot)} \\
%              \cline{2-13} 
%              Method & \multicolumn{12}{c}{Sessions} \\
%              \cline{2-13} 
%               &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
%              \midrule
%              GAT\_finetune  &0.866&0.059&0.069&0.059&0.020&0.018&0.031&0.023&0.018&0.031&0.119&0.834  \\
%              GAT\_frozen  &0.867&0.841&0.821&0.793&0.775&0.760&0.745&0.725&0.712&0.699&0.773&0.169 \\            
%              SAVC  &0.862&0.845&0.835&0.808&0.794&0.777&0.763&0.746&0.728&0.711&0.787&0.151 \\
%              TAP &0.873&0.854&0.837&0.819&0.805&0.793&0.779&0.765&0.752&0.742&0.802&0.131 \\
%             \midrule


\section{Generalizability for Session Size}
To evaluate the impact of session size on TAP's performance, we conducted experiments varying the number of incremental sessions from 5 to 20. To deepen our understanding of this effect, we present the final session accuracy across base classes, novel classes, and all classes, respectively. The results reveal a strengthening trend in TAP's overall performance, with gains of 1.9\%, 4.4\%, 3.9\%, and 8.7\% over GAT-frozen as the number of sessions increases. For the base classes, GAT-frozen, which maintains a fixed backbone, slightly outperforms TAP. However, in the novel classes, TAP demonstrates significant improvements of 8\%, 12\%, 12.3\%, and 12.4\% over GAT-frozen. This indicates that TAP favors enhanced performance in extended sessions. Notably, TAP consistently achieves stable performance gains in novel classes regardless of session size.
When the number of sessions is limited, the prevalence of base classes in the test set tends to dominate overall performance. Conversely, as the number of sessions increases, the contribution of novel classes to the final performance becomes more significant, thereby highlighting TAP's advantage.
\begin{table*}[h]
% \vspace{-0.3cm}
    \centering
    \caption{Performance comparison with regard to varying number of sessions on the Amazon\_clothing dataset (3-way 5-shot).}
    % \vspace{-0.2cm}
    \scalebox{0.6}{
    \begin{tabular}{ccccc|cccc|cccc}
         \toprule
        & \multicolumn{4}{c}{All classes} &\multicolumn{4}{c}{Base classes} &\multicolumn{4}{c}{Novel classes} \\
        \cline{2-13} 
        & \multicolumn{12}{c}{Number of total sessions (\#)} \\
        \cline{2-13} 
         Methods & \#5  & \#10  & \#15  & \#20 & \#5  & \#10  & \#15  & \#20 & \#5  & \#10  & \#15  & \#20 \\
         \midrule
         GAT-frozen &0.762&0.703&0.680&0.545 &0.812&0.847&0.849&0.903 &0.473&0.478&0.516&0.439 \\
         SAVC & 0.780 & 0.738 & 0.652 & 0.539 & 0.805 & 0.839 & 0.845 & 0.914 &0.592 & 0.554 & 0.508 & 0.428  \\
         TAP &0.781&0.747&0.719&0.632 &0.811&0.846&0.827&0.862 &0.553&0.593&0.639&0.563 \\
    \bottomrule
    \end{tabular}}
    \label{table:perf_stats}
    \vspace{-0.3cm}
\end{table*}

\section{Performance Relation to the Structural Statistics}

Table \ref{table:perf_stats} presents the potential influence of dataset statistics on model performance. It summarizes TAP's improvements of the last session accuracy over GAT\_frozen, alongside key dataset characteristics, \ie average node degree and graph homophily rate. The benchmark datasets exhibit a range of statistics, with edge density varying from 6.59 to 14.14 and homophily rates ranging from 0.29 to 0.72. Considering both performance and dataset statistical properties, TAP demonstrates strong robustness and generalizability, maintaining consistent performance across diverse datasets. Specifically, TAP does not show evident sensitivity on the average node degree, but it is more likely to achieve superior results on datasets with higher homophily rates, as evidenced by over 7.0\% improvements on Amazon\_clothing and Cora\_full compared to 4.8\% on DBLP. %In cases where the homophily rate is low, TAP tends to perform better on denser graph datasets than on sparser ones.
\begin{table*}[h]
% \vspace{-0.3cm}
    \centering
    \caption{Performance comparison with regard to dataset statistics of Average degree and homophily rate.}
    \vspace{-0.2cm}
    \scalebox{0.8}{
    \begin{tabular}{ccccc}
         \toprule
         Methods & Amazon\_clothing  & DBLP  & Cora\_full  & Ogbn-arxiv \\
         \midrule
         Average degree & 7.35 & 14.14 & 6.59 & 13.7  \\
         Homophily rate & 0.62 & 0.29 & 0.59 & 0.72  \\
         Improvements & 0.077 & 0.048 & 0.070 & 0.058  \\
    \bottomrule
    \end{tabular}}
    \label{table:perf_stats}
    \vspace{-0.3cm}
\end{table*}

\section{Experimental Results for N-way 1-shot Setting}
%To further elaborate on the performance of TAP on the N-way 1-shot setting, we provide specific experimental results in Table \ref{table:1-shot} as the complementary for Figure \ref{fig:1-shot} in Section \ref{sec:1-shot}. As observed in the table, in terms of the last session accuracy, TAP achieves improvements of 2.0\%, 4.5\%, 3.6\% and 3.9\% on Ogbn-arxiv, Amazon\_clothing, DBLP and Cora\_full, respectively, compared with the best baselines. The stable performance improvements demonstrate the strong robustness of TAP against the overfitting risk caused by the extremely label-sparsity problem.
To further elaborate on TAP’s performance in the N-way 1-shot setting, we present specific experimental results in Table \ref{table:1-shot}, which complement Figure \ref{fig:1-shot} in Section \ref{sec:1-shot}. As shown in the table, TAP achieves improvements of 2.0\%, 4.5\%, 3.6\%, and 3.9\% in the final session accuracy on the Ogbn-Arxiv, Amazon\_Clothing, DBLP, and Cora\_Full datasets, respectively, compared to the best baselines. These consistent performance improvements demonstrate TAP’s strong robustness against the overfitting risk associated with extreme label sparsity.
\begin{table*}[th]
\vspace{-0.1cm}
    \centering
    \tabcolsep 3pt
    \caption{Performance comparison on the N-way 1-shot setting over different datasets.}
   \vspace{-0.3cm}
    \scalebox{0.6}{
        \begin{tabular}{l c c c c c c c c c c c c}
             \toprule
              & \multicolumn{12}{c}{Obgn-arxiv (3-way 1-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.668&0.482&0.270&0.183&0.141&0.089&0.081&0.084&0.061&0.056 &0.211 &0.612  \\
             GAT\_frozen  &0.662&0.579&0.538&\underline{0.491}&0.437&0.414&0.392&\underline{0.362}&0.346&0.323&0.454 &0.339 \\
             CLOM\cite{zou2022margin} &0.654&0.576&0.532&0.481&0.427&0.402&0.383&0.353&0.340&0.316 &0.446 &\underline{0.338} \\
             LCWOF\cite{kukleva2021generalized} &0.666&0.586&0.544&0.489&0.435&0.411&0.391&\underline{0.362}&\underline{0.348}&\underline{0.324}&\underline{0.455} &0.341   \\
             Alice\cite{peng2022few}  &0.654&0.572&0.537&0.487&0.434&0.406&0.386&0.345&0.332&0.310 &0.446 &0.344 \\
             SAVC\cite{song2023learning}  &\underline{0.674}&\underline{0.589}&\underline{0.549}&0.490&\underline{0.439}&\underline{0.416}&\underline{0.393}&0.349&0.336&0.313 &0.454 &0.361 \\
             NC-FSCIL\cite{yang2023neural} &0.658&0.490&0.395&0.391&0.384&0.360&0.331&0.303&0.292&0.287 &0.389 &0.371\\
             Geometer\cite{peng2022few} &0.661&0.579&0.538&\underline{0.491}&0.437&0.414&0.392&0.361&0.346&0.323 &{0.454} &0.338\\
             \rowcolor{LightCyan} \textbf{TAP} &\textbf{0.669}&\textbf{0.599}&\textbf{0.565}&\textbf{0.513}&\textbf{0.462}&\textbf{0.433}&\textbf{0.410}&\textbf{0.378}&\textbf{0.366}&\textbf{0.344} &\textbf{0.474} &\textbf{0.325} \\
            \midrule
             & \multicolumn{12}{c}{Amazon\_clothing (5-way 1-shot)}\\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions} \\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.931&0.082&0.061&0.026&0.051&0.078&0.091&0.056&0.037&0.022 &0.143 &0.909\\
             GAT\_frozen  &0.931&0.825&0.778&0.714&0.669&0.612&0.574&0.552&0.531&0.511 &0.669 &0.420\\
             CLOM\cite{zou2022margin}  &0.943&\underline{0.836}&0.775&0.723&0.674&0.615&0.578&0.555&0.533&0.511 &0.675 &0.432 \\
             LCWOF\cite{kukleva2021generalized} &0.931&0.817&0.766&0.707&0.658&0.603&0.567&0.544&0.523&0.500  &0.662 &0.431\\
             Alice\cite{peng2022few}  &0.935&0.832&0.778&0.729&\underline{0.677}&0.620&0.582&0.555&0.535&0.513 &0.675 &0.422 \\
             SAVC\cite{song2023learning}  &0.924&0.836&0.778&\underline{0.735}&\underline{0.677}&\underline{0.621}&0.585&0.558&0.535&0.518 &0.677 &\underline{0.406}\\
             NC-FSCIL\cite{yang2023neural} &0.835&0.709&0.622&0.580&0.504&0.479&0.426&0.424&0.427&0.372&0.538 &0.463\\
             Geometer\cite{peng2022few} &\underline{0.944}&0.832&\underline{0.781}&0.720&\underline{0.677}&0.619&\underline{0.589}&\underline{0.566}&\underline{0.545}&\underline{0.520} &\underline{0.679} &0.423\\
             \rowcolor{LightCyan} \textbf{TAP} &\textbf{0.934}&\textbf{0.837}&\textbf{0.783}&\textbf{0.743}&\textbf{0.703}&\textbf{0.652}&\textbf{0.629}&\textbf{0.605}&\textbf{0.585}&\textbf{0.565} &\textbf{0.703} &\textbf{0.369}\\
             \midrule             
             & \multicolumn{12}{c}{DBLP (10-way 1-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions}\\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9 & Average Acc.  & PD \textcolor{red}{$\downarrow$} \\
             \midrule
             GAT\_finetune  &0.638&0.225&0.113&0.089&0.073&0.065&0.054&0.051&0.043&0.041 &0.139 &0.597 \\
             GAT\_frozen  &0.632&0.595&0.567&0.540&0.512&0.485&0.464&0.444&0.426&0.412 &0.507 &0.220 \\
             CLOM\cite{zou2022margin}  &0.645&0.607&0.575&0.544&0.516&0.489&0.468&0.448&0.432&0.417 &0.514 &0.228 \\
             LCWOF\cite{kukleva2021generalized}  &0.628&0.591&0.559&0.531&0.503&0.478&0.457&0.437&0.420&0.408 &0.501 &0.220 \\
             Alice\cite{peng2022few}  &0.616&0.590&0.563&0.536&0.514&0.490&0.471&0.453&\underline{0.436}&0.422 &0.509 &0.194 \\
             SAVC\cite{song2023learning}  &0.608&0.589&0.564&0.541&0.518&\underline{0.495}&\underline{0.473}&\underline{0.454}&\underline{0.436}&\underline{0.423} &0.509 &\underline{0.185} \\
             NC-FSCIL\cite{yang2023neural} &0.430&0.319&0.296&0.298&0.282&0.277&0.286&0.260&0.244&0.243&0.293 &0.187\\
             Geometer\cite{peng2022few} &\underline{0.653}&\underline{0.613}&\underline{0.579}&\underline{0.547}&\underline{0.519}&0.491&0.469&0.447&0.428&0.415 &\underline{0.516} &0.238\\
             \rowcolor{LightCyan} \textbf{TAP} &\textbf{0.642}&\textbf{0.616}&\textbf{0.592}&\textbf{0.567}&\textbf{0.545}&\textbf{0.522}&\textbf{0.501}&\textbf{0.486}&\textbf{0.469}&\textbf{0.459}  &\textbf{0.540} &\textbf{0.183}\\
            \midrule
             & \multicolumn{12}{c}{Cora\_full (5-way 1-shot)} \\
             \cline{2-13} 
             Method & \multicolumn{12}{c}{Sessions}\\
             \cline{2-13} 
              &0& 1 &2 & 3 &4 &5 &6 & 7 &8 & 9  & Average Acc.  & PD \textcolor{red}{$\downarrow$}  \\
             \midrule
             GAT\_finetune  &0.937&0.104&0.075&0.052&0.051&0.047&0.042&0.039&0.041&0.036 &0.142 &0.901\\
             GAT\_frozen  &\underline{0.946}&0.813&\underline{0.711}&\underline{0.645}&{0.567}&0.529&0.487&{0.455}&0.426&0.401 &0.598 &0.544\\
             CLOM\cite{zou2022margin}  &0.943&0.812&\underline{0.711}&0.641&\underline{0.572}&\underline{0.532}&\underline{0.490}&\underline{0.458}&0.432&0.402 &\underline{0.599} &0.540\\
             LCWOF\cite{kukleva2021generalized} &0.938&0.799&0.695&0.625&0.554&0.511&0.473&0.445&0.420&0.392 &0.585 &0.545\\
             Alice\cite{peng2022few}  &0.941&0.796&0.691&0.625&0.558&0.516&0.472&0.445&0.420&0.394 &0.586 &0.546\\
             SAVC\cite{song2023learning}  &0.939&0.786&0.680&0.607&0.539&0.499&0.458&0.430&0.405&0.375 &0.571 &0.564\\
             NC-FSCIL\cite{yang2023neural} &0.897&0.672&0.632&0.575&0.507&0.466&0.438&0.417&0.397&0.366 &0.537 &0.531\\
             Geometer\cite{peng2022few} &0.938& \underline{0.815}& {0.697}& 0.631& 0.567& 0.531& 0.486& 0.452& \underline{0.435}& \underline{0.411} &0.596 &\underline{0.526}\\
             \rowcolor{LightCyan} \textbf{TAP} &\textbf{0.944}&\textbf{0.838}&\textbf{0.747}&\textbf{0.682}&\textbf{0.621}&\textbf{0.579}&\textbf{0.538}&\textbf{0.506}&\textbf{0.480}&\textbf{0.450} &\textbf{0.638} &\textbf{0.493}\\
             \bottomrule 
        \end{tabular}}
    \label{table:1-shot}
\end{table*}


